An evaluation approach to computing invariants rings of permutation groups

Using evaluation at appropriately chosen points, we propose a Gr\"obner basis free approach for calculating the secondary invariants of a finite permutation group. This approach allows for exploiting the symmetries to confine the calculations into a smaller quotient space, which gives a tighter control on the algorithmic complexity, especially for large groups. This is confirmed by extensive benchmarks using a Sage implementation.

==> benchmark-canonics-linear.tex <==
  \begin{tikzpicture}[xscale=1.5, yscale=0.9]
    \tikzstyle{bull}=[minimum size=4pt, inner sep=0pt] 
    \tikzstyle{vertical}=[very thin, color=gray] 
    \tikzstyle{degree}=[thin] 
    \tikzstyle{horizontal}=[-, color=gray] 
      % axis 
      \draw[->] (0,0) -- (7.0,0); 
      \draw[->] (0,0) -- (0,7.8); 

      \draw (7.3, 0) node[right] {$C(G)$}; 
      %\draw (0, 8.1) node[above] {$\text{time}$}; 

      \draw[dashed, color=red] (0, 0.3) -- (6.5, 7.6);

\draw[vertical] (0.301029995663981,-0.1) -- (0.301029995663981,7.8);
\draw[vertical] (0.778151250383644,-0.1) -- (0.778151250383644,7.8);
\draw[vertical] (1.38021124171161,-0.1) -- (1.38021124171161,7.8);
\draw[vertical] (2.07918124604762,-0.1) -- (2.07918124604762,7.8);
\draw[vertical] (2.85733249643127,-0.1) -- (2.85733249643127,7.8);
\draw[vertical] (3.70243053644553,-0.1) -- (3.70243053644553,7.8);
\draw[vertical] (4.60552052343747,-0.1) -- (4.60552052343747,7.8);
\draw[vertical] (5.55976303287679,-0.1) -- (5.55976303287679,7.8);
\draw[vertical] (6.55976303287679,-0.1) -- (6.55976303287679,7.8);


\draw[horizontal] (-0.1, 1.00000000000000) -- (7.0, 1.00000000000000);
\draw[horizontal] (-0.1, 2.00000000000000) -- (7.0, 2.00000000000000);
\draw[horizontal] (-0.1, 3.00000000000000) -- (7.0, 3.00000000000000);
\draw[horizontal] (-0.1, 4.00000000000000) -- (7.0, 4.00000000000000);
\draw[horizontal] (-0.1, 5.77815125038364) -- (7.0, 5.77815125038364);
\draw[horizontal] (-0.1, 7.55630250076729) -- (7.0, 7.55630250076729);

\draw (-0.2, 1.00000000000000) node[left] {$10^{-3}s$};
\draw (-0.2, 2.00000000000000) node[left] {$10^{-2}s$};
\draw (-0.2, 3.00000000000000) node[left] {$10^{-1}s$};
\draw (-0.2, 4.00000000000000) node[left] {$1s$};
\draw (-0.2, 5.77815125038364) node[left] {$1min$};
\draw (-0.2, 7.55630250076729) node[left] {$1h$};

      \draw (0.301, -0.2) node[below] {$2!$};
      \draw (0.778, -0.2) node[below] {$3!$};
      \draw (1.380, -0.2) node[below] {$4!$};
      \draw (2.079, -0.2) node[below] {$5!$};
      \draw (2.857, -0.2) node[below] {$6!$};
      \draw (3.702, -0.2) node[below] {$7!$};
      \draw (4.605, -0.2) node[below] {$8!$};
      \draw (5.559, -0.2) node[below] {$9!$};
      \draw (6.559, -0.2) node[below] {$10!$};

\draw (4.29939833006815, 5.28782024147230) node[bull] {$\bullet$};
\draw (3.13225968953104, 3.72921985299736) node[bull] {$\bullet$};
\draw (2.41161970596323, 3.06103808726086) node[bull] {$\bullet$};
\draw (3.74919504221967, 4.51888976071329) node[bull] {$\bullet$};
\draw (4.05300157040031, 4.71592440815311) node[bull] {$\bullet$};
\draw (5.63027935550066, 6.53980552346748) node[bull] {$\bullet$};
\draw (3.71197585435176, 4.62441771860681) node[bull] {$\bullet$};
\draw (5.00756856255847, 5.72924989132721) node[bull] {$\bullet$};
\draw (5.12624508203868, 6.24502040963965) node[bull] {$\bullet$};
\draw (5.13231413306668, 6.29213502385141) node[bull] {$\bullet$};
\draw (5.81738421049044, 6.68882421014052) node[bull] {$\bullet$};
\draw (4.43901672838751, 5.44154680627729) node[bull] {$\bullet$};
\draw (4.12635872706927, 4.82295061846088) node[bull] {$\bullet$};
\draw (2.58546072950850, 3.04464919359928) node[bull] {$\bullet$};
\draw (3.15533603746506, 4.46069821302106) node[bull] {$\bullet$};
\draw (3.82859545637170, 4.65233299650394) node[bull] {$\bullet$};
\draw (4.76075410950582, 5.57093575348835) node[bull] {$\bullet$};
\draw (4.27698998936823, 4.84391159791995) node[bull] {$\bullet$};
\draw (3.68601029131528, 4.53573187121855) node[bull] {$\bullet$};
\draw (5.96888436862963, 6.79224710549411) node[bull] {$\bullet$};
\draw (3.99056082999402, 4.69192855192569) node[bull] {$\bullet$};
\draw (2.39794000867204, 3.01222526967731) node[bull] {$\bullet$};
\draw (1.62324929039790, 2.26629983151499) node[bull] {$\bullet$};
\draw (5.83512911292975, 6.66781104964826) node[bull] {$\bullet$};
\draw (4.65616530635089, 5.51996140911308) node[bull] {$\bullet$};
\draw (2.63245729218472, 3.71568162519675) node[bull] {$\bullet$};
\draw (2.41161970596323, 3.04142803924536) node[bull] {$\bullet$};
\draw (4.17960923372620, 4.80504934789983) node[bull] {$\bullet$};
\draw (5.63235098332215, 6.53387089421459) node[bull] {$\bullet$};
\draw (3.75243260926147, 4.64712378217416) node[bull] {$\bullet$};
\draw (4.82604239145547, 5.57337582109499) node[bull] {$\bullet$};
\draw (4.01456253812761, 4.76067997174290) node[bull] {$\bullet$};
\draw (5.11837386483425, 6.33768523329226) node[bull] {$\bullet$};
\draw (4.58515605250508, 5.52894115126058) node[bull] {$\bullet$};
\draw (4.13548249133571, 4.80371563072429) node[bull] {$\bullet$};
\draw (2.12057393120585, 3.01350290148405) node[bull] {$\bullet$};
\draw (0.000000000000000, 0.403055479293754) node[bull] {$\bullet$};
\draw (4.07162429853975, 4.77593825612505) node[bull] {$\bullet$};
\draw (5.23657756537085, 6.29400617945879) node[bull] {$\bullet$};
\draw (3.61320735210376, 4.57477912140838) node[bull] {$\bullet$};
\draw (0.698970004336019, 1.24996247441770) node[bull] {$\bullet$};
\draw (4.76475132232462, 5.58761928342968) node[bull] {$\bullet$};
\draw (4.27362620627296, 4.85008759551901) node[bull] {$\bullet$};
\draw (1.14612803567824, 1.98050612804511) node[bull] {$\bullet$};
\draw (5.16177814191687, 6.30579936025652) node[bull] {$\bullet$};
\draw (5.77309716865631, 6.66346225790192) node[bull] {$\bullet$};
\draw (5.17416160628806, 5.86821471551043) node[bull] {$\bullet$};
\draw (4.12577394985088, 4.82473686102874) node[bull] {$\bullet$};
\draw (4.22520586596590, 5.99938477787301) node[bull] {$\bullet$};
\draw (5.57761242044122, 6.53951262260633) node[bull] {$\bullet$};
\draw (4.84954839300348, 5.63596324775413) node[bull] {$\bullet$};
\draw (2.95760728706009, 3.81247273721235) node[bull] {$\bullet$};
\draw (5.15214151579703, 6.33557779750827) node[bull] {$\bullet$};
\draw (4.18067055295789, 4.80791489886814) node[bull] {$\bullet$};
\draw (5.11837386483425, 6.34137713059168) node[bull] {$\bullet$};
\draw (5.81738421049044, 6.69811985789013) node[bull] {$\bullet$};
\draw (1.23044892137827, 1.89030450525493) node[bull] {$\bullet$};
\draw (5.24062412018726, 6.31804682487703) node[bull] {$\bullet$};
\draw (5.01749661795356, 5.72281711693313) node[bull] {$\bullet$};
\draw (4.01004541263610, 4.74988420925596) node[bull] {$\bullet$};
\draw (2.46389298898591, 3.10081136562604) node[bull] {$\bullet$};
\draw (1.67209785793572, 2.36739465626141) node[bull] {$\bullet$};
\draw (4.12952877385878, 5.26944108995977) node[bull] {$\bullet$};
\draw (5.93237938669689, 6.73372963248061) node[bull] {$\bullet$};
\draw (4.38553477891021, 5.39437328853437) node[bull] {$\bullet$};
\draw (2.40823996531185, 3.05523344203814) node[bull] {$\bullet$};
\draw (4.16334030561825, 4.82417302872976) node[bull] {$\bullet$};
\draw (3.73567872590590, 4.58140415903393) node[bull] {$\bullet$};
\draw (3.54431614174743, 4.53164876886553) node[bull] {$\bullet$};
\draw (0.698970004336019, 1.20574217388401) node[bull] {$\bullet$};
\draw (4.94609348000589, 5.68274483893090) node[bull] {$\bullet$};
\draw (4.12319807503200, 4.80130284820922) node[bull] {$\bullet$};
\draw (5.96888436862963, 6.79637428206125) node[bull] {$\bullet$};
\draw (4.43771886133624, 5.45771792444391) node[bull] {$\bullet$};
\draw (4.03734680356809, 4.75126424114426) node[bull] {$\bullet$};
\draw (2.41161970596323, 3.05686701439368) node[bull] {$\bullet$};
\draw (5.82102590166929, 6.68831620275156) node[bull] {$\bullet$};
\draw (3.15533603746506, 4.48882954592846) node[bull] {$\bullet$};
\draw (5.57761242044122, 6.53929963766389) node[bull] {$\bullet$};
\draw (4.62811293764317, 5.50497428384068) node[bull] {$\bullet$};
\draw (2.12057393120585, 3.00755941831652) node[bull] {$\bullet$};
\draw (4.80954624793092, 5.56549625132036) node[bull] {$\bullet$};
\draw (4.27742583227586, 4.84423417281265) node[bull] {$\bullet$};
\draw (5.49880109834536, 6.49066684419852) node[bull] {$\bullet$};
\draw (4.00766244653728, 4.75815433428519) node[bull] {$\bullet$};
\draw (5.72579732923296, 6.58516652224616) node[bull] {$\bullet$};
\draw (5.18744739220121, 5.83733814181806) node[bull] {$\bullet$};
\draw (3.94205768384139, 4.70231187292703) node[bull] {$\bullet$};
\draw (2.51719589794997, 3.06994116789619) node[bull] {$\bullet$};
\draw (3.68681495450732, 5.14285986949801) node[bull] {$\bullet$};
\draw (5.40077622478663, 6.42840481701115) node[bull] {$\bullet$};
\draw (5.86854746059986, 6.68237778667015) node[bull] {$\bullet$};
\draw (4.63339775072268, 5.48586657885349) node[bull] {$\bullet$};
\draw (2.63245729218472, 3.74571252881110) node[bull] {$\bullet$};
\draw (0.301029995663981, 0.758093866196314) node[bull] {$\bullet$};
\draw (4.09694475517694, 4.73606079921932) node[bull] {$\bullet$};
\draw (6.14496100881373, 6.89348368181697) node[bull] {$\bullet$};
\draw (3.73295636957562, 4.60570780377941) node[bull] {$\bullet$};
\draw (5.13697092756359, 5.81070409591459) node[bull] {$\bullet$};
\draw (4.01089331310438, 4.75314026663915) node[bull] {$\bullet$};
\draw (1.85733249643127, 2.40706873640669) node[bull] {$\bullet$};
\draw (6.15122271075079, 6.90326358268396) node[bull] {$\bullet$};
\draw (4.49213153358157, 5.43462804259297) node[bull] {$\bullet$};
\draw (3.37254380075907, 3.91703894750513) node[bull] {$\bullet$};
\draw (2.14921911265538, 2.99271666811409) node[bull] {$\bullet$};
\draw (4.05679054827438, 4.70555037253598) node[bull] {$\bullet$};
\draw (5.25684036996316, 6.31659009433359) node[bull] {$\bullet$};
\draw (3.61352470285365, 4.57568883377499) node[bull] {$\bullet$};
\draw (4.73930329915634, 5.55661459638800) node[bull] {$\bullet$};
\draw (4.26237988807736, 4.85444991354014) node[bull] {$\bullet$};
\draw (4.22520586596590, 5.85306345982988) node[bull] {$\bullet$};
\draw (1.14612803567824, 1.94234919960501) node[bull] {$\bullet$};
\draw (5.40377404580975, 6.41002027113143) node[bull] {$\bullet$};
\draw (5.72668891120169, 6.59249101505016) node[bull] {$\bullet$};
\draw (4.47274182636120, 5.40997249722664) node[bull] {$\bullet$};
\draw (4.13519627960660, 4.80467722696758) node[bull] {$\bullet$};
\draw (2.57170883180869, 3.08694667374988) node[bull] {$\bullet$};
\draw (3.81277970700896, 4.58601154544293) node[bull] {$\bullet$};
\draw (5.60566267991018, 6.55741848959171) node[bull] {$\bullet$};
\draw (4.67710485173431, 5.48563728250447) node[bull] {$\bullet$};
\draw (4.24664627489071, 4.86013038361816) node[bull] {$\bullet$};
\draw (5.70171042409954, 6.62329357188265) node[bull] {$\bullet$};
\draw (1.23044892137827, 1.89298878910005) node[bull] {$\bullet$};
\draw (5.83329057758008, 6.69780664886598) node[bull] {$\bullet$};
\draw (4.84516628092834, 5.54546148031934) node[bull] {$\bullet$};
\draw (3.88047059280378, 4.63712561399898) node[bull] {$\bullet$};
\draw (2.51719589794997, 3.06275128624701) node[bull] {$\bullet$};
\draw (1.62324929039790, 2.58285842412944) node[bull] {$\bullet$};
\draw (5.24062412018726, 6.30800834818623) node[bull] {$\bullet$};
\draw (3.67200544502295, 4.50954270796008) node[bull] {$\bullet$};
\draw (4.63007174996866, 5.51410703131193) node[bull] {$\bullet$};
\draw (3.39269695325966, 3.88420269850337) node[bull] {$\bullet$};
\draw (2.39794000867204, 3.02703509388405) node[bull] {$\bullet$};
\draw (4.16163748070459, 4.78783628727344) node[bull] {$\bullet$};
\draw (5.63438556489254, 6.54751570249015) node[bull] {$\bullet$};
\draw (3.63103769653674, 4.52509004253554) node[bull] {$\bullet$};
\draw (4.86621051830032, 5.65128092338634) node[bull] {$\bullet$};
\draw (4.01287938717129, 4.75888064844368) node[bull] {$\bullet$};
\draw (5.13231413306668, 6.30979491457427) node[bull] {$\bullet$};
\draw (6.16206381327365, 6.88344250853734) node[bull] {$\bullet$};
\draw (4.41747169320329, 5.42779794029439) node[bull] {$\bullet$};
\draw (4.03454824709847, 4.73844186973157) node[bull] {$\bullet$};
\draw (2.31386722036915, 3.03905342115367) node[bull] {$\bullet$};
\draw (3.30297993674825, 4.42689561207724) node[bull] {$\bullet$};
\draw (5.60810972436897, 6.55859357870656) node[bull] {$\bullet$};
\draw (3.60260252042026, 4.55226901811770) node[bull] {$\bullet$};
\draw (3.68681495450732, 5.16475944105527) node[bull] {$\bullet$};
\draw (4.79813940997493, 5.55526230257645) node[bull] {$\bullet$};
\draw (4.27694408571298, 4.84992147559153) node[bull] {$\bullet$};
\draw (3.81378107817408, 4.58284711451189) node[bull] {$\bullet$};
\draw (5.83692955329364, 6.70883714979680) node[bull] {$\bullet$};
\draw (5.18673320101394, 5.83409720919505) node[bull] {$\bullet$};
\draw (3.87771680086498, 4.57852059205005) node[bull] {$\bullet$};
\draw (2.58994960132571, 3.05874144933852) node[bull] {$\bullet$};
\draw (5.80612364776578, 6.74009609385030) node[bull] {$\bullet$};
\draw (5.57888665294113, 6.53549029197405) node[bull] {$\bullet$};
\draw (4.41785350516848, 5.32376601699328) node[bull] {$\bullet$};
\draw (3.08707120590654, 3.78255442227360) node[bull] {$\bullet$};
\draw (4.10195317747720, 4.72598054033614) node[bull] {$\bullet$};
\draw (5.11837386483425, 6.34023675206956) node[bull] {$\bullet$};
\draw (5.63748772815084, 6.55688071884162) node[bull] {$\bullet$};
\draw (1.23044892137827, 1.93180502629740) node[bull] {$\bullet$};
\draw (5.15666119333417, 5.83220014782286) node[bull] {$\bullet$};
\draw (4.13519627960660, 4.80901849645459) node[bull] {$\bullet$};
\draw (1.83884909073726, 2.49429301277118) node[bull] {$\bullet$};
\draw (6.16291641870391, 6.88057603677830) node[bull] {$\bullet$};
  \end{tikzpicture} 

